Tracking System Behaviour from Resource Usage Data

Resource usage data, collected using tools such as TACC Stats, capture the resource utilization by nodes within a high performance computing system. We present methods to analyze the resource usage data to understand the system performance and identify performance anomalies. The core idea is to model the data as a three-way tensor corresponding to the compute nodes, usage metrics, and time. Using the reconstruction error between the original tensor and the tensor reconstructed from a low rank tensor decomposition, as a scalar performance metric, enables us to monitor the performance of the system in an online fashion. This error statistic is then used for anomaly detection that relies on the assumption that the normal/routine behavior of the system can be captured using a low rank approx- imation of the original tensor. We evaluate the performance of the algorithm using information gathered from system logs and show that the performance anomalies identified by the proposed method correlates with critical errors reported in the system logs. Results are shown for data collected for 2013 from the Lonestar4 system at the Texas Advanced Computing Center (TACC)

==> methods.tex <==
\subsection{Background - Tensor Decomposition}
One reason for using a tensor based representation of the resource usage data is to be able to exploit the correlations among the different modes in the data. For instance, several usage metrics (See Table~\ref{tab:metrics}) are expected to exhibit a correlated structure. Similarly, one would expect a temporal regularity in the data and correlations across different computational nodes. 
We exploit the presence of these structures by employing tensor decomposition methods to express the data in terms of lower rank factorization of the tensor. We employ these methods to make future predictions based on historical data, and then compare it with observed data to obtain an error metric. Two of the most widely used tensor decomposition methods are: the CANDECOMP/PARAFAC or CP method~\cite{CEM:CEM582} and Tucker decomposition~\cite{Tucker1966}. 
%In this paper, we use the CP method for tensor decomposition, which works as follows:
Both CP and Tucker methods are higher order generalizations of the widely used Singular Value Decomposition (SVD) and Principal Component Analysis (PCA), respectively. We provide brief description of the two methods here.
\subsubsection{Tucker Tensor Decomposition}
The Tucker decomposition~\cite{Tucker1966} is a higher order generalization of PCA and involves decomposition of a tensor into a lower rank core tensor, multiplied by a matrix along each mode as illustrated in Figure~\ref{fig:tucker}.
\begin{defn}
  Let $\mathcal{T}$ be a tensor of size $M\times N \times T$. A rank-($M',N',T'$) Tucker decomposition of $\mathcal{T}$ yields a core tensor $\mathcal{G}$ of size $M'\times N' \times T'$ and three factor matrices (usually orthogonal), ${\bf A}_M$, ${\bf A}_N$, and ${\bf A}_T$, of sizes $M \times M'$, $N \times N'$, and $T \times T'$, respectively, such that:
  \begin{equation}
  \widehat{\mathcal{T}} \approx \mathcal{G} \times {\bf A}_M \times {\bf A}_N \times {\bf A}_T
    \label{eqn:tucker}
  \end{equation}
  \label{defn:tucker}
\end{defn}
$(M',N',T')$ are also referred to as the $n$-{\em rank} of the tensor.
\input{tensortucker}
The core tensor and the factor matrices capture the level of interaction between different modes. The Tucker decomposition is typically computed by solving the following optimization problem:
\begin{equation}
    \underset{\mathcal{G},{\bf A}_M,{\bf A}_N,{\bf A}_T}{\min} \Vert\mathcal{T} - \mathcal{G} \times {\bf A}_M \times {\bf A}_N \times {\bf A}_T\Vert_F^2
    \label{eqn:tuckeropt}
\end{equation}
where $\Vert\Vert_F$ is the {\em Frobenius norm} of the matrix.
The most popular approach to solve the above formulation is the {\em higher order orthogonal iteration} (HOOI) method, which uses the leading singular vectors of the matricized tensor along each mode to compute the factor matrices in an iterative fasion.
\subsubsection{CANDECOMP/PARAFAC (CP) Tensor Decomposition}
The CP decomposition~\cite{CEM:CEM582} method treats the tensor as a sum of finite number of rank one tensors (See Figure~\ref{fig:cp}).
\begin{defn}
  Let $\mathcal{T}$ be a tensor of size $M\times N\times K$. A rank-$R$ CP decomposition of $\mathcal{T}$ yields $R$ arrays for each mode, such that:
  \begin{equation}
    \mathcal{T} \approx \sum_{i=0}^{R}\lambda_i\times({\bf a}_{Mi}\circ {\bf a}_{Ni} \circ {\bf a}_{Ti})
    %\underset{\mathcal{T},{\bf a},{\bf b},{\bf c}}{\min} \Vert\mathcal{T} - \sum_{i=0}^{n}\lambda_i\times(a_i\circ b_i \circ c_i)\Vert_F^2
    \label{eqn:cp}
  \end{equation} 
  where $\circ$ denotes the outer vector product. $R$ is referred to as the {\em rank} of the tensor.
  \label{defn:cp}
\end{defn}
For a given rank, $R$, computing the CP decomposition is typically done using an {\em Alternating Least Squares} (ALS) approach that minimizes the following objective function:
\begin{equation}
  \underset{\mathcal{T},A_M,A_N,A_T}{\min} \Vert\mathcal{T} - \sum_{i=0}^{n}\lambda_i\times({\bf a}_{Mi}\circ {\bf a}_{Ni} \circ {\bf a}_{Ti})\Vert_F^2
  \label{eqn:cpopt}
\end{equation} 
where the vectors ${\bf a}_{Mi}, {\bf a}_{Ni}, {\bf a}_{Ti}$ are the $i^{th}$ columns of the matrices $A_M,A_N,A_T$, respectively.
\input{tensorcp}
\subsection{Approximation Error using Tucker Tensor Decomposition}
The recovered tensor in~\eqref{}
\subsection{Using Tucker Tensor Decomposition to Compute a Tracking Metric}
Our focus is on predicting the resource usage metrics at a given time instance $t$, using historical data, which is then compared to the observed data to obtain the desired error metric, as discussed in the beginning of this section. Given the historical tensor $\mathcal{T}_{i:t-1}$, we predict the time-slice at $t$, i.e, $T_t$. We make an assumption of temporal locality, i.e., the behavior at $t$ will only depend on a finite history and not on the entire history so far. Thus, we make the predictions at $t$ a $k$ length sub-tensor, $\mathcal{T}_{t-k:t-1}$.
\subsubsection{Using Tucker Decomposition}
\input{tuckeralgo}
This method uses Tucker decomposition to predict the future values. The idea is to create an augmented tensor at time $t$, that consists of the historical $K$ length window from $\mathcal{T}$ and the future time slice (or multiple slices), appended at the end. The appended values are initialized to the mean value for each resource usage metric. By computing the lower rank tensor decomposition of this augmented tensor and then recreating the approximated tensor, we ``fill'' the unknown values for future time slices by exploiting the relationships across the three modes. The predicted values are compared to the observed data to compute the error metric. The steps of the proposed algorithm are outlined in Algorithm~\ref{alg:tuckererror}. The input parameters to this algorithm include the data tensor, $\mathcal{T}$, the lower rank along each mode used for Tucker decomposition, the window size, $K$, and the number of slices to be predicted at a given time instance, $L$. If $L=1$, then only one time slice is predicted using the previous $K$ length window. By taking higher values of $L$, the algorithm produces error metric at a coarser resolution. Experimental results show that higher values of $L$ produce less noisy output, while reducing the computational complexity of the algorithm by a factor of $L$.
We initialize the desired matrix $\overline{T}_t$ with the corresponding mean values for the corresponding metric, i.e., $\overline{T}_t[m,n] = \mu_m$, where $\mu_m$ is equal to the mean value for the $m^{th}$ resource usage metric. The initialized tensor is appended to the end of $\mathcal{T}_{t-k:t-1}$ to obtain an augmented $M \times N \times (k+1)$ tensor, $\mathcal{T}'_{t-k:t}$. We then apply Tucker decomposition on $\mathcal{T}'_{t-k:t-1}$ (See Definition~\ref{defn:tucker}) to obtain a $M' \times N' \times k'$ core tensor and the corresponding factor matrices. These are used to reconstruct the approximate sub-tensor, $\widehat{\mathcal{T}'}_{t-k:t}$, using~\eqref{eqn:tucker}. The $t^{th}$ time slice of $\widehat{\mathcal{T}'}_{t-k:t}$ is used as the predicted time slice, $\overline{T}_t$. 

The error metric at time $t$, denoted by $\epsilon_t$, is calculated as:
\begin{equation}
  \epsilon_t = \Vert\overline{T_t} - T_t\Vert_F
  \label{eqn:error1}
\end{equation}

In this method we use historical data to predict the future behavior of the system. The predicted output is then compared with the observed data to identify anomalies. This method relies on the assumption that the system exhibits a stable behavior along the time dimension in a local sense, when performing normally. Let $\mathcal{T}_t$ denote the sub-tensor corresponding to the $K$ length window starting at time instance $t$. Predicting future tensor portion specified as $L$ length $\mathcal{T}_{t+l}^{L}$ starting at $t+l$ time instance $l$ . This part includes no information related to any part of tensor, it is a filling empty sub-tensor. That missing data could be generated using {\em recreate} the $K+L$ where $K>>L$ length sub-tensor $\mathcal{T}_{t}^{K+L}$ starting at time instance $t$ could be subject to ${predict}$  $\widetilde{\mathcal{T}}_{t}^{K+L}$ starting at time instance $t$ and length $K+L$. The evaluated sub-tensor part $\widetilde{\mathcal{T}}_{l}^{L}$ could be compared with the $\mathcal{T}_{l}^{L}$ tensor. The frobenius norm of the difference is close to 

\begin{equation}
  \gamma_t = \Vert\widetilde{\mathcal{T}}_{l} - {\mathcal{T}}_{l}\Vert_F
  \label{eqn:method3}
\end{equation}
\subsubsection{Using CP Decomposition}
\input{cpalgo}
We use the components extracted by the CP model (See Definition~\ref{defn:cp}) from the historical sub-tensor, $\mathcal{T}_{t-K:t-1}$ to predict the time slice at time $t$, $T_t$. Recall that for CP, the outer product ${\bf a}_{Mi}{\bf b}_{Ni}^\top$ between the vectors ${\bf a}_{Mi}$ and ${\bf a}_{Ni}$, captures the relationship between the metrics and the nodes in the $i^{th}$ component while the temporal behavior is captured in the vector ${\bf a}_{Ti}$. We combine the contribution of each of the $R$ outer products (where $R$ is the rank of the tensor) by using the temporal profiles, according to the following formula:
\begin{equation}
  \widehat{T}_t = \sum_{i = 1}^R \gamma_i\lambda_i{\bf a}_{Mi}{\bf a}_{N_i}^\top
\end{equation}
where,
\begin{equation}
\gamma_i = \frac{1}{z}\sum_{k = 0}^{K-1}e^{-\rho(K-k-1)}{\bf a}_{Ti}[t-K+k]\text{, where, }z = \sum_{k=0}^{K-1}e^{-\rho(K-k-1)}
\label{eqn:gamma}
\end{equation}
$\rho$ is a scalar constant specified as an input parameter. The effect of the exponential term in~\eqref{eqn:gamma} is to weight the historical information by its recency, i.e., the effect of more recent observations in time should be more than older information. The scalar constant $\rho$ controls the rate at which the weight ``decays'' with time. Larger values of $\rho$ result in treating only the most recent temporal values as important. Smaller values of $\rho$ means that data from older time instances have a significant impact on the prediction. If $\rho=0$, every time instance in the window has equal effect on the prediction.

A similar approach has been previously suggested for link prediction in temporal web data~\cite{Dunlavy:2011:TLP:1921632.1921636}. However, the previous work assumes a constant dependence on previous time steps, instead of the exponential weighting scheme proposed here. 
The final error is computed by computing the Frobenius norm between the predicted and true matrices at time $t$. The steps of the CP based algorithm are given in Algorithm~\ref{alg:cperror}.

The computational complexity of the decomposition step (line 4) in Algorithm~\ref{alg:cperror} is $O(MNK)$ per iteration of the ALS routine. The number of iterations depends on the nature of the data. For $\nu$ average iterations, the overall complexity of the entire algorithm is $O(\nu MNT)$, i.e., it scales linearly with the size of the raw data along each mode. The storage requirements are also bound by the size and rank of the tensor, i.e., $O(R(M +N +T))$.


==> tuckeralgo.tex <==
\begin{algorithm}
  \begin{algorithmic}[1]
    \Function{TuckerDecomp}{$\mathcal{T} \in \mathbb{R}^{M\times N \times T}, M',N',T',K,L$}
    \State ${\bm \epsilon} \leftarrow \{\}$
    \State $t \leftarrow k+1$\Comment{Start after first window}
    \While{$t \le T$}
    \State $\mathcal{P} \leftarrow Zeros(M,N,L)$
    \For{$m = 1$ to $M$}
    \State $\mathcal{P}[m,:,:] \leftarrow \mu_m$\Comment{Mean value for $m^{th}$ metric}
    \EndFor
    \State $\mathcal{Q} \leftarrow rightappend(\mathcal{T}_{t-K:t-1},\mathcal{P})$
    \State $\mathcal{G},A_M,A_N,A_T \leftarrow Tucker(\mathcal{Q},M',N',T')$\Comment{See~\eqref{eqn:tuckeropt}}
    \State $\widehat{\mathcal{Q}} \leftarrow \mathcal{G}\times A_M \times A_N \times A_T$
    \State ${\bm \epsilon}[t] \leftarrow \Vert\widehat{\mathcal{Q}}_{t:t+l} - \mathcal{T}_{t:t+l}\Vert_F$
    \State $t \leftarrow t + L$
    \EndWhile
    \\
    \Return ${\bm \epsilon}$
    \EndFunction

  \end{algorithmic}
  \caption{Tucker decomposition based monitoring}\label{alg:tuckererror}
\end{algorithm}

